Vector-Valued Least-Squares Regression under Output Regularity Assumptions

We propose and analyse a reduced-rank method for solving least-squares regression problems with infinite dimensional output. We derive learning bounds for our method, and study under which setting statistical performance is improved in comparison to full-rank method. Our analysis extends the interest of reduced-rank regression beyond the standard low-rank setting to more general output regularity assumptions. We illustrate our theoretical insights on synthetic least-squares problems. Then, we propose a surrogate structured prediction method derived from this reduced-rank method. We assess its benefits on three different problems: image reconstruction, multi-label classification, and metabolite identification.

==> proofs/crossterm.tex <==
In this subsection we bound the cross-term appearing in the  decomposition $\eqref{eq:comp}$:
\begin{align}
    \E_x[\|(\hat P - P)(\hat h(x) - h^*(x))\|^2_{\bmY}]
\end{align}
\lemcross*
\begin{proof} We have
\begin{align}
    \E[\|(\hat P - P)(\hat h(x) - h^*(x))\|^2_{\bmY}]^{1/2} &= \|(\hat P - P)(H_n-H)S^*\|_{\text{HS}}\\
    &\leq A \times B
\end{align}
with
\begin{align}
    A &= \|(\hat P - P)(HCH^* + t)^{1/2}\|_{\text{HS}}\\
    B &= \|(HCH^* + t)^{-1/2}(H_n-H)S^*\|_{\text{HS}}
\end{align}
Then, using the Lemma \ref{lem:set}, if $t \geq c_5n^{-\frac{1}{\beta + \nu + 2\alpha}}$ with $\xi=\frac{1}{14}$, with probability at least $1-3\delta$ we have
\begin{align}
    A &=  \|(\hat P - I + I - P)(HCH^* + t)^{1/2}\|_{\text{HS}}\\
    &\leq \|(\hat P - I)(HCH^* + t)^{1/2}\|_{\text{HS}} + \|(I - P)(HCH^* + t)^{1/2}\|_{\text{HS}}\\
    &\leq \sqrt{3}\sqrt{\mu_{p+1}(M) + t} + \sqrt{\mu_{p+1}(M) + t}\\
    &\leq 3\sqrt{\mu_{p+1}(M) + t}
\end{align}
Then, from Theorem B.8 in \citep{ciliberto2020general} we get, as in proof of Lemma \ref{lem:HnC-H},
\begin{align*}
    B \leq \quad & \frac{8\kappa \log \frac{2}{\delta}}{\sqrt{\lambda}n} \times (Q + \kappa c_1c_2 t^{-\frac{1}{2} (\beta + \alpha)})\\
    &+ \frac{8\kappa}{\sqrt{n}} \times \sqrt{(\lambda^{-1} \times  c_1c_4t^{-(\nu + \alpha)} + c_1c_2 t^{-(\beta + \alpha})\log \frac{4}{\delta}}\\
    &+ 10 \times \lambda^{1/2} c_1c_2 t^{-\frac{1}{2} (\beta + \alpha)}
\end{align*}
So, if $\lambda = \max\left(\frac{1}{n}, \frac{\|PE^{1/2}\|_{\text{HS}}}{\sqrt{n}}\right)$, and taking $t=\mu_{p+1}(M)$, we have
\begin{align*}
    A \times B \leq& \frac{24\kappa \log \frac{2}{\delta}}{n^{1/2}} \times \sqrt{2}(Q\mu_{p+1}(M)^{1/2} + \kappa c_1c_2 \mu_{p+1}(M)^{1/2(1-(\beta + \alpha))})\\
    &+ 24\kappa\log \frac{4}{\delta} \times n^{-1/4} \left(\|E^{1/2}\|_{\infty}^{-1/2} \times c_1c_4 \mu_{p+1}(M)^{1/2(1-(\nu + \alpha))} + n^{-1/4}c_1c_2\mu_{p+1}(M)^{1/2(1-(\beta + \alpha))}\right)\\
    &+ 30 \times n^{-1/4} \|E^{1/2}\|_{\text{HS}}^{1/2} \times c_1c_2 \mu_{p+1}(M)^{1/2(1-(\beta + \alpha))}\\
    &\leq 30(c_1(c_2+c_4))n^{-1/4}\log(4/\delta)\big(\frac{\kappa}{\|E^{1/2}\|_{\infty}^{1/2}} \mu_{p+1}(M)^{1/2(1-(\nu + \alpha))} + \|E^{1/2}\|_{\text{HS}}^{1/2} \mu_{p+1}(M)^{1/2(1-(\beta + \alpha))}\\
    &\quad + \mathcal{O}(n^{-1/4})\big)
\end{align*}
We define $\epsilon(p) = 30(c_1(c_2+c_4))\left(\frac{\kappa}{\|E^{1/2}\|_{\infty}^{1/2}} \mu_{p+1}(M)^{1/2(1-(\nu + \alpha))} + \|E^{1/2}\|_{\text{HS}}^{1/2} \mu_{p+1}(M)^{1/2(1-(\beta + \alpha))} + \mathcal{O}(n^{-1/4})\right) $.

We get the wanted upper bound.
\end{proof}

==> sections/discussion.tex <==
\textbf{Plateau threshold.} When bounding $\E[\|\hat P h^*(x) - h^*(x)\|_{\bmY}^2]^{\frac{1}{2}}$ a plateau threshold $p^*$ appears such that the bound remains constant w.r.t $p$ for $p > p^*$. This plateau can be defined with $\mu_p(M) \leq t^*$, with $t^*$ decreasing with $n$. When $\mu_p(M) \leq t^*$, the bound is
\begin{align}
    \E[\|\hat P h^*(x) - h^*(x)\|_{\bmY}^2]^{\frac{1}{2}} \leq 3 \mathcal{N}_{M}(t)^{\frac{1}{2}} \sqrt{\mu_p(M) + t}
\end{align}
with $\mathcal{N}_{M}(t) = \Tr(M(M+t)^{-1})$, $M=HCH^*, h^*(.)=H\phi(.), C=\E[\phi(x) \otimes \phi(x)]$.

\textbf{Assumption 3. } There exists $\beta \in [0,1/2]$ such that
\begin{align}
    \|(ZZ^* + t)^{-\frac{1}{2}}H\|_{\infty} \lesssim \frac{1}{t^{\beta}}
\end{align}
and because of Assumption 1 we have $Z^*=HS^*$, so
\begin{align}
    \|(HCH^* + t)^{-\frac{1}{2}}H\|_{\infty} \lesssim \frac{1}{t^{\beta}}
\end{align}

\textbf{Role of assumption 3.} Assumption 3 allows to bound the following crucial quantity w.r.t $t$ and $\lambda$
\begin{align}
    \|(M+t)^{-\frac{1}{2}} H (C + \lambda)^{-\frac{1}{2}}\|_{\hs}
\end{align}
and thereby to get fast divergence rate w.r.t $n$ of the plateau threshold $p^*$ to $+ \infty$ (see below). In general, without this assumption, we have $t^* \sim \E[\|\hat h(x) - h^*(x)\|^2_{\bmY}]$, which leads to
\begin{align}
    \E[\|\hat h(x) - h^*(x)\|^2_{\bmY}]^{\frac{1}{2}} = o(\E[\|\hat P h^*(x) - h^*(x)\|_{\bmY}^2]^{\frac{1}{2}}).
\end{align}
That is the minimal reconstruction error is bigger than the regression error for $p=p^*$, thus for all $p\in \mathbb{N}^*$. In this case there is no possible gain with our reduced-rank estimator.

\textbf{Input and output regularity. } Let $A \in \bmH_x \otimes \bmH_x$, $C \in \bmY \otimes \bmY$ be two positive semidefinite operators.  Then, the following condition
\begin{align}
    \|(A+t)^{-1} H (C+t)^{-1}\|_{\hs} \lesssim \frac{1}{t^{\alpha}}\frac{1}{\lambda^{\beta}}
\end{align}
is verified by all operators of the form
\begin{align}
    H = A^{1-\alpha}H_0C^{1-\beta}
\end{align}
with $\|H_0\|_{\hs} < +\infty$. Now, doing the singular value decomposition $H_0=\sum\limits_{i=1}^{+\infty} \mu_i u_i \otimes v_i$, we have
\begin{align}
    H = \sum\limits_{i=1}^{+\infty} \mu_i (A^{1-\alpha} u_i) \otimes (C^{1-\beta} v_i)
\end{align}
showing that $A$ requires each $u_i \in \bmY$ to have fast decreasing coefficients in the basis of the main components of $A$. Similarly, $C$ requires each $v_i \in \bmH_x$ to have fast decreasing coefficients in the basis of the main components of $C$.
 
 
\textbf{Rank one example. } If we consider the rank one case where there are $y_0 \in \bmY$ and $h_0 \in \bmH_x$ such that
\begin{align}
    H = y_0 \otimes h_0
\end{align}
then
\begin{align}
    \|M_t^{-\frac{1}{2}} H C_{\lambda}^{-\frac{1}{2}}\|_{\hs} &= \Tr(M_t^{-\frac{1}{2}} y_0 \otimes h_0 C_{\lambda}^{-1} h_0 \otimes y_0 M_t^{-\frac{1}{2}})^{\frac{1}{2}}\\
    &= \langle h_0,\, C_{\lambda}^{-1}h_0\rangle^{\frac{1}{2}} \langle y_0,\, M_{t}^{-1}y_0\rangle^{\frac{1}{2}}
\end{align}
Moreover, because $M = HCH^*$, we have
\begin{align}
    \langle y_0,\, M_{t}^{-1}y_0\rangle &= \langle y_0,\, (HCH^* + t)^{-1}y_0\rangle\\
    &= \langle y_0,\, (\langle h_0,\,Ch_0\rangle y_0 \otimes y_0 + t)^{-1}y_0\rangle\\
    &= \frac{\|y_0\|^2}{\langle h_0,\,Ch_0\rangle \|y_0\|^2 + t}\\
    &\leq \frac{1}{\langle h_0,\,Ch_0\rangle}
\end{align}
So, for any $C, y_0, h_0$, we have
\begin{align}
    \|M_t^{-\frac{1}{2}} H C_{\lambda}^{-\frac{1}{2}}\|_{\hs} &\leq \frac{\langle h_0,\, C_{\lambda}^{-1}h_0\rangle^{\frac{1}{2}}}{\langle h_0,\,Ch_0\rangle^{\frac{1}{2}}}
\end{align}
\begin{figure}[ht!]
\centering
\includegraphics[width=0.4\linewidth]{figures/rankoneex.pdf}
\caption{$\|M_t^{-\frac{1}{2}} H C_{\lambda}^{-\frac{1}{2}}\|_{\hs}$ w.r.t $t$ and $\lambda$. Assumption 3 numerical verification with rank one example. log scale. }
\end{figure}

\textbf{Finite rank $H$. } When $H$ is finite rank the assumption 3 holds with $\beta=0$ (best case). Indeed, let be $H \in \bmY \otimes \bmH_x$ with finite rank $r$, then $H$ can be written
\begin{align}
    \sum\limits_{i=1}^r \mu_i y_i\otimes h_i
\end{align}
with $\mu_i \in \R$, $y_i \in \bmY$, $h_i \in \bmH_x$. Hence, we also have:
\begin{align}
    HCH^* = \sum\limits_{i,j=1}^r \mu_i \mu_j \langle h_i,\, C h_j\rangle y_i \otimes y_j.
\end{align}
Then
\begin{align}
    \|(HCH^* + t)^{-\frac{1}{2}}H\|_{\hs}^2 &= \Tr((HCH^* + t)^{-1}HH^*)\\
\end{align}
We note $A: V \rightarrow V$ and $B: V \rightarrow V$ the restrictions of the operator $HH^*$ and $HCH^*$ to $V:= \spn(y_1, \dots, y_r)$. $B$ has only strictly positive eigenvalues as $\langle h_k,\, Ch_k\rangle >0$ for all $k \in \llbracket 1, k \rrbracket$.
So, for all $t>0$,
\begin{align}
    \Tr((HCH^* + t)^{-1}HH^*) &=  \Tr((B + t)^{-1}A)\\
    &\leq \|A\|_{\hs}^2 \|(B + t)^{-1}\|_{\infty}\\
    &\leq \frac{\|H\|_{\hs}^2}{\mu_r(B)}
\end{align}

\textbf{Alternative Assumption 3. } There exists $\alpha > 0 $ and $\beta \in [0, \frac{1}{2}]$, $A$ a positive semidefinite operators from $\bmY$ to $\bmY$, such that
\begin{align}
    H = AH_0C^{\beta}
\end{align}
with $\|H_0\|_{\hs} < +\infty$ and
\begin{align}
    A^{\alpha} \preceq H_0C^{2\beta+1}H_0^*.
\end{align}
In this case we have:
\begin{align}
    \|(M+t)^{-\frac{1}{2}} H (C + \lambda)^{-\frac{1}{2}}\|_{\hs} &\leq t^{-\frac{1}{2} \frac{\alpha}{2 + \alpha}} \lambda^{-\frac{1}{2}(1-2\beta)}.
\end{align}

\textbf{Example. } For any $H_0 \in \bmY \otimes \bmH_x$, choose $A = \left(H_0CH_0^*\right)^{2}$, then the alternative assumption holds with $\alpha = \frac{1}{2}$, and $\beta = 0$.



\textbf{Assumption 3 - $t^*$ convergence rate. } When the problem is such that, there exist $\alpha, \beta \in [0, \frac{1}{2}]$, with
\begin{align}
    \|(M+t)^{-\frac{1}{2}} H (C + \lambda)^{-\frac{1}{2}}\|_{\hs} \lesssim \frac{1}{t^{\alpha}}\frac{1}{\lambda^{\beta}}
\end{align}
one can show that
\begin{align}
    t^* \sim n^{-\frac{1-\beta}{\alpha + (1-\beta)}}
\end{align}
in comparison to 
\begin{align}
    \E[\|\hat h(x) - h^*(x)\|^2_{\bmY}] \sim n^{-\frac{1-\beta}{\frac{1}{2} + (1-\beta)}}
\end{align}
if $\| H (C + \lambda)^{-\frac{1}{2}}\|_{\hs} \lesssim \frac{1}{\lambda^{\beta}}$.

% In the following Table are given examples of learning rates for $t^*$ depending on $\alpha, \beta$.
% \begin{table}[!ht]
%   \centering
%   \begin{tabular}{lll}
%     \toprule
%     $\alpha$ / $\beta$ & $0$ & $\frac{1}{2}$ \\
%     \midrule
%      $0$ & $n^{-1}$ & $n^{-1}$ \\
%      $\frac{1}{2}$  & $n^{-\frac{2}{3}}$ & $n^{-\frac{1}{2}}$\\
%     \bottomrule
%   \end{tabular}
% \caption{$t^*$ rate w.r.t $\alpha, \beta \in [0, \frac{1}{2}]$}
% \label{notations}
% \end{table}

\textbf{Standard source condition. } The source condition can be written as the existence of $\beta>0$ and $H_0 \in \bmY \otimes \bmH_x$ with $\|H_0\|_{\hs} < + \infty$ such that
\begin{align}
    H = H_0 C^{\beta}
\end{align}
this implies
\begin{align}
    \|HC_{\lambda}^{-\frac{1}{2}}\|_{\hs} &\leq \frac{1}{\lambda^{(\frac{1}{2} - \beta)_+}}
\end{align}
which lead to an improved rate of the kernel ridge estimator. We can check how the source condition also improve the convergence rate of $t^*$. We have, for any $\gamma \in [0, \beta]$
\begin{align}
    \|M_t^{-\frac{1}{2}} H C_{\lambda}^{-\frac{1}{2}}\|_{\infty} &= \|(H_0C^{2\beta+1}H_0^* + t)^{-\frac{1}{2}} H_0 C^{\beta} C_{\lambda}^{-\frac{1}{2}}\|_{\infty}\\
    &\leq \|(H_0C^{2\beta+1}H_0^* + t)^{-\frac{1}{2}} H_0 C^{\gamma}\|_{\infty} \times \|C^{\beta - \gamma}C_{\lambda}^{-\frac{1}{2}}\|_{\infty}\\
    &\leq \|(H_0C^{2\beta+1}H_0^* + t)^{-\frac{1}{2}} H_0 C^{2\gamma}H_0^*(H_0C^{2\beta+1}H_0^* + t)^{-\frac{1}{2}}\|_{\infty}^{\frac{1}{2}} \times \lambda^{-\frac{1}{2}+ (\beta-\gamma)}
\end{align}
but:
\begin{align}
    H_0 C^{2\gamma}H_0^* &= H_0 C^{2\beta +1 \times \frac{2\gamma}{2\beta +1}}H_0^* \preceq \|H_0\|_{\infty}^{2 - \frac{4\gamma}{2\beta + 1}} \times (H_0 C^{2\beta +1}H_0^*)^{\frac{2\gamma}{2\beta +1}}
\end{align}
so, noting $A = H_0 C^{2\beta +1}H_0^*$, and $b = \|H_0\|_{\infty}^{2 - \frac{4\gamma}{2\beta + 1}}$ we have
\begin{align}
    \|(H_0C^{2\beta+1}H_0^* + t)^{-\frac{1}{2}} H_0 C^{2\gamma}H_0^*(H_0C^{2\beta+1}H_0^* + t)^{-\frac{1}{2}}\|_{\infty}^{\frac{1}{2}} &\leq b \|(A + t)^{-\frac{1}{2}} A^{\frac{2\gamma}{2\beta +1}} (A + t)^{-\frac{1}{2}}\|_{\infty}^{\frac{1}{2}}\\
    &\leq b \times \left(\sup_i \frac{\mu_i(A)^{\frac{2\gamma}{2\beta +1}}}{\mu_i(A) + t}\right)^{\frac{1}{2}}\\
    &\leq b \times t^{-\frac{1}{2}(1-\frac{2\gamma}{2\beta +1})}
\end{align}
using $x^ay^{1-a} \leq x + y$ for any $x,y \in \R^+, a \in [0,1]$.

Now, in order to balance the different terms in the proof of convergence of $t^*$, we compute $\lambda$ such that
\begin{align}
    \frac{1}{\sqrt{\lambda n t}} = \lambda^{-\frac{1}{2}+ (\beta-\gamma)} \times t^{-\frac{1}{2}(1-\frac{2\gamma}{2\beta +1})}
\end{align}
and we obtain
\begin{align}
    \frac{1}{\sqrt{\lambda n t}} = t^{\frac{1}{2}(\frac{\gamma}{(2\beta+1)(1+\beta-\gamma))} -1)} \times n^{-\frac{1}{2}(1-\frac{1}{2(1 +\beta - \gamma)})}
\end{align}
then choosing $t$ such that $\frac{1}{\sqrt{\lambda n t}} \leq 1$ we obtain the rate of $t^*$
\begin{align}
    t^* &= n^{\frac{(2\beta+1)(1/2 + \beta - \gamma)}{(2\beta+1)(1+\beta-\gamma) - \gamma}}\\
    &= n^{\frac{\beta + 1/2}{\beta +1}}
\end{align}
then $\sqrt{t}$ in the reconstruction error bound has the same rate than the kernel ridge estimator under the same assumption. Notice that the rate of $t^*$ finally doesn't depend on the chosen $\gamma \in [0, \beta]$.

\textbf{Source condition with $\beta > \frac{1}{2}$. } If $\beta > \frac{1}{2}$ the rate of $\sqrt{t^*}$ is strictly better than $n^{-\frac{1}{3}}$ which is the rate of the ridge estimator under the same assumption. Hence, this is a sufficient assumption for showing a gain with the proposed estimator.

\textbf{Interpretation of Assumption 3. } Assumption 3 can be interpreted as requiring that the main components of $H$ are identifiable thanks to the main components of $HCH^* = \E[h^*(x) \otimes h^*(x)]$. 

==> sections/experiments.tex <==
\subsection{Synthetic Experiments}

In this subsection we illustrate our theoretical results on synthetic least-squares problems.

\textbf{Synthetic least-squares with various output source condition.} For $d=200$, we generate $C \in \R^{d \times d}$ with $\mu_p(C) = \frac{1}{p^{2}}$, and random eigenvectors $(v_p)_{p=1}^d$ defined by an orthogonal matrix $V \in \R^{d \times d}$ drawn from the Haar distribution. We generate $H_0 \in \R^{d \times d}$ with independently drawn coefficients from the standard normal distribution. We compute $\|(M + t)^{-\frac{1}{2}}H\|_{\infty}^2$ w.r.t $t$ with $H=(H_0CH_0^*)^{\gamma}H_0$ for various $\gamma \in [0, 1.5]$. We plot the results in Figure \ref{fig:source_cond} (left) in log-log scale, with the slopes $\beta = \frac{1}{2\gamma + 1}$. We compute and plot on Figure \ref{fig:source_cond} (right) $\|H(C+\lambda)^{-\frac{1}{2}}\|_{\infty}^2$ w.r.t $\lambda$. Firstly, we see that the Assumption \ref{as:3} indeed improved when $\gamma$ increases, while the source condition does not change. We know that $H = (H_0CH_0^*)^{\gamma}H_0$ verifies Assumption \ref{as:3} with $\beta = \frac{1}{2\gamma + 1}$, but depending on $H_0$ it might be verified with $\beta \ll \frac{1}{2\gamma + 1}$. Nonetheless, notice that with our generated $H_0$, $\beta = \frac{1}{2\gamma + 1}$ are sharp for the associated $H =  (H_0CH_0^*)^{\gamma}H_0$. 

 \begin{figure}[ht]
\begin{minipage}[b]{0.5\linewidth}\centering
\includegraphics[width=70mm]{figures/source_cond.pdf}
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}\centering
\includegraphics[width=70mm]{figures/output_source_cond.pdf}
\end{minipage}
\caption{Source condition $\|H(C + \lambda)^{-\frac{1}{2}}\|_{\infty}^2$ w.r.t $\lambda$ (left) and output source condition $\|(M + t)^{-\frac{1}{2}}H\|_{\infty}^2$ (right) in log-log scale for $H=(H_0CH_0^*)^{\gamma}H_0$ and various $\gamma \in \{0, 0.1, 0.25, 0.5, 0.9, 1.5\}$.}
\label{fig:source_cond}
\end{figure}

\textbf{Dataset generation. } For $d=250$, $\bmX = \bmH_x = \bmY = \R^d$, we choose the target eigenvalues $\left(\mu_k(h^*)\right)_{k=1}^d$ and the noise eigenvalues $\left(\mu_k(\epsilon)\right)_{k=1}^d$ (finite rank or exponential decay). Then, we generate $n_{train}= 500, n_{test}=1000$ couples $(x,y)$ such that $x \sim \mathcal{N}(0, I_{\bmY})$, and $y = Hx + \epsilon$ with $H : \bmX \rightarrow \bmY$ such that $\mu_k(HH^T) = \mu_k(h^*)$ and $\mu_k(\E[\epsilon \otimes \epsilon])= \mu_k(\epsilon)$. We draw randomly the eigenvector associated to each eigenvalue.

\textbf{Experiments. } On the Figure \ref{fig:exp} we compare our method with the unsupervised learning of $\hat P$ via $
    \min\limits_{P \in\mathcal{P}_p} \frac{1}{n}\sum\limits_{i=1}^n \|P y_i - y_i\|^2_{\bmY}$, and with the optimal projection defined by $\min\limits_{P \in\mathcal{P}_p} \E[\|Ph^*(x) - h^*(x) \|^2_{\bmY}]$, for different values of $p$. We select the parameter $\lambda_1$ using 5-Folds cross-validation minimizing $\frac{1}{n}\sum\limits_{i=1}^n \|\hat h_{\lambda_1}(x_i) - y_i\|^2_{\bmY}]$, and $\lambda_2$ by 5-Folds cross-validation minimizing $\frac{1}{n}\sum\limits_{i=1}^n \| \hat h_{\lambda_2}(x_i) - \hat P y_i\|^2_{\bmY}$. Then, we compute the test MSE on the test set.

\textbf{Comments on the results. } We see that the MSE of our estimator is improved (for well-chosen $p$) in comparison to the kernel ridge estimator. We also see that our estimator's performance is close to the one using the optimal projection. Moreover, we see that using unsupervised subspace learning do not lead to a gain. These experiments confirm the interest of our estimator when output regularity assumptions are verified.

\begin{figure}[ht!]
\centering
\begin{minipage}{.3\textwidth}
    \centering
    \includegraphics[width=1.1\linewidth]{figures/synth_oel_finiterank.pdf}
\end{minipage}
\hfil
\begin{minipage}{.3\textwidth}
    \centering
    \includegraphics[width=1.1\linewidth]{figures/synth_oel_finiterank_mse.pdf}
\end{minipage}
\hfil
\begin{minipage}{.3\textwidth}
    \centering
    \includegraphics[width=1.1\linewidth]{figures/synth_oel_finiterank_lambda.pdf}
\end{minipage}

\begin{minipage}{.3\textwidth}
    \centering
    \includegraphics[width=1.1\linewidth]{figures/synth_oel_expdecay.pdf}
\end{minipage}
\hfil
\begin{minipage}{.3\textwidth}
    \centering
    \includegraphics[width=1.1\linewidth]{figures/synth_oel_expdecay_mse.pdf}
\end{minipage}
\hfil
\begin{minipage}{.3\textwidth}
    \centering
    \includegraphics[width=1.1\linewidth]{figures/synth_oel_expdecay_lambda.pdf}
\end{minipage}
\caption{Synthetic experiments. $P$ is the optimal projection. $\hat P_s$ is the projection estimated with supervised subpace learning. $\hat P_u$ is the projection estimated with unsupervised subpace learning. $\hat h$ is the KRR estimator. $\hat h_{denoised}$ is the KRR estimator trained with denoised data $(x, h^*(x))$. Upper/bottom left: Signal/noise setup. Upper/bottom middle: test MSE w.r.t $p$. Upper/bottom right: selected $\lambda_2$ w.r.t $p$ (with 5-fold cross-validation).}
\label{fig:exp}
\end{figure}


